Achieving High Throughput with a Trainable Neural-Network-Based Equalizer for Communications on FPGA

The ever-increasing data rates of modern communication systems lead to severe distortions of the communication signal, imposing great challenges to state-of-the-art signal processing algorithms. In this context, neural network (NN)-based equalizers are a promising concept since they can compensate for impairments introduced by the channel. However, due to the large computational complexity, efficient hardware implementation of NNs is challenging. Especially the backpropagation algorithm, required to adapt the NN's parameters to varying channel conditions, is highly complex, limiting the throughput on resource-constrained devices like field programmable gate arrays (FPGAs). In this work, we present an FPGA architecture of an NN-based equalizer that exploits batch-level parallelism of the convolutional layer to enable a custom mapping scheme of two multiplication to a single digital signal processor (DSP). Our implementation achieves a throughput of up to 20 GBd, which enables the equalization of high-data-rate nonlinear optical fiber channels while providing adaptation capabilities by retraining the NN using backpropagation. As a result, our FPGA implementation outperforms an embedded graphics processing unit (GPU) in terms of throughput by two orders of magnitude. Further, we achieve a higher energy efficiency and throughput as state-of-the-art NN training FPGA implementations. Thus, this work fills the gap of high-throughput NN-based equalization while enabling adaptability by NN training on the edge FPGA.

==> chapters/design_space_exploration.tex <==
\section{Design Space Exploration}
\label{sec:dse}

An optimized neural network topology is crucial for hardware implementation of \ac{ann}-based algorithms, as it has a huge influence on the power consumption, throughput, and latency of the final implementation. However, the design of efficient \acp{ann} topologies is characterized by an enormous design space with various hyperparameters. This design space includes the layer type, the number of layers, the size of each layer, the activation function, and multiple more hyperparameters. An exploration of all those parameters is nearly infeasible, thus we restrict our analysis to the topology template presented in the following, which provides sufficient configurability while comprising a manageable design space.  

\subsection{\ac{cnn} Topology Template}
\label{sec:topology}

The core of our equalizer is a one-dimensional \ac{cnn} since it resembles the structure of traditional convolutional filters. The \ac{cnn} is based on a customizable topology template shown in Fig. \ref{fig:network_topology}, where specific parameters are determined in an extensive design space exploration. 

\begin{figure}[b!]
    \vspace{-4mm}
	\centerline{\input{figures/tikz_topology.tex}}
	\caption{Topology template of the equalizer \ac{cnn}. The feature map dimensions are given next to the arrows, where the first dimension corresponds to the number of channels and the second one to the width.}
 	\label{fig:network_topology}
\end{figure}


The \ac{cnn} is composed of $L$ convolutional layers with similar kernel size $K$ and padding $P$. Each convolutional layer but the last is followed by batch normalization and \ac{relu} activation functions. One channel is used for the input sequence, while subsequent activations consist of $C$ channels. The output of the \ac{cnn} is based on $V_\mathrm{p}$ channels, thus $V_\mathrm{p}$ values are calculated in parallel for one pass of the network. To shift the input sequence accordingly, the first layer has a stride of $V_\mathrm{p}$, while the following layers have a stride of one, and the last stride is set corresponding to the oversampling factor $N_\mathrm{os}$. 
After the last convolutional layer, the feature map is flattened so that each element of the feature map corresponds to one output symbol. Afterwards, the output is mapped to the closest constellation symbol. 

\subsection{Design Space Exploration Framework}

To explore this design space, we design a framework that allows to automatically evaluate multiple configurations, which are compared in terms of communication performance and complexity. Further, the framework features cross-layer analysis by providing an estimation of the achievable throughput. Thus hardware metrics are already included in the topology search, which greatly reduces the development cycles since multiple models can already be discarded in an early design phase. 

As configurable hyperparameters of the \ac{cnn}, we select the number of layers $L$, the kernel size $K$, the number of channels $C$, and the symbols calculated in 
parallel $V_p$. We train each configuration three times for \num{10000} iterations with a learning rate of \num{0.001} with Adam optimizer and \ac{mse} loss. 
After training, the highest achieved \ac{ber} of the three training runs and the corresponding \ac{mac} operations per input symbol of each configuration are determined by our framework. This way, a trade-off between communication performance and hardware complexity can be found. 

\subsection{Quantization}
\label{sec:quant}

In addition to the network topology, another essential aspect of an efficient \ac{ann} implementation on resource-constrained devices is the quantization of weights and activations. In contrast to the \num{32}-bit floating-point format used in software, each value is represented in fixed-point format with arbitrary decimal and fraction width on the \ac{fpga}. 

To explore the quantization efficiently, we include an automated quantization approach in our framework, similar to the one proposed in \cite{nikolic2020}. Therefore, the loss function is modified to simultaneously learn the precision of each layer while optimizing the accuracy of the \ac{ann} during training. This is achieved by using a differentiable interpolation of the bit-widths, which allows to train them using backpropagation. Similar to \cite{nikolic2020}, we include a trade-off factor in the loss function, which determines how aggressively to quantize. This enables efficient exploration of the trade-off between bit width and communication performance. %In contrast to \cite{nikolic2020} -- where an integer representation together with a scaling factor that is coupled to the bit-width of the values is learned -- we adjust the algorithm to separately learn the integer and fraction width. This way, there is no need to scale the values in hardware during computation, as the numbers are directly represented by their corresponding fixed-point value and can directly be mapped to our hardware architecture. 
%With the help of our framework, we perform a quantization analysis for the most promising candidates found in the first step of the design space exploration. 


\subsection{Results of Design Space Exploration}

In Fig. \ref{fig:dse}, the results of the design space exploration are shown. Our design space is spanned by the following four dimensions: symbols calculated in parallel  $V_p \in \mlrb{1, 2, 4, 8, 16}$, network depth $L \in \mlrb{3, 4, 5}$, kernel size $K \in \mlrb{9, 15, 21}$ and the number of channels $C \in \mlrb{3, 4, 5}$. Thus, overall \num{135} different models are trained and evaluated. The average \ac{mac} operations per symbol $\mathrm{MAC}_\mathrm{sym}$ can be calculated as follows: 
\begin{equation*}
    \mathrm{MAC}_\mathrm{sym} = \frac{K \cdot C}{V_p} + (L - 2) \cdot \frac{K \cdot C \cdot C}{V_p} + \frac{K \cdot C}{V_p \cdot N_\mathrm{os}} \; .
\end{equation*}


\begin{figure}[b!]
	\centering
	%\vspace*{0.18cm}
	\input{figures/tikz_dse.tex}
	\caption{Results of design space exploration of the \ac{cnn} topology. The maximal $\mathrm{MAC}_\mathrm{sym}$ to achieve the throughput of \SI{40}{\giga Bd} is given by the vertical red lines for different frequencies, while the baseline \ac{ber} is given by the horizontal red line.}
        %\vspace*{-4mm}
	\label{fig:dse}
\end{figure}

In Fig. \ref{fig:dse} each $V_p$ is illustrated with a different color, to highlight its influence on accuracy and complexity. 
For comparison, we also give the \ac{ber} of a conventional adaptive linear equalizer based on the Sato algorithm \cite{Sato1975} with 40 taps. To ensure that our \ac{ann}-based equalizer outperforms the conventional one, we define the linear equalizer's \ac{ber} as our baseline, which is given by the red horizontal line. Pareto optimal models are shown by the black dotted line. Further, the framework approximates the maximal $\mathrm{MAC}_\mathrm{sym}$ to achieve the required throughput $T_\mathrm{req}$ of \SI{40}{\giga Bd} based on the clock frequency $f_\mathrm{clk}$, and the available \acp{dsp} of our target device as follows: 
\begin{equation*}
   \mathrm{MAC}_\mathrm{sym, max} = \frac{\mathrm{DSP}_\mathrm{avail}}{T_\mathrm{req}} \cdot f_\mathrm{clk} \cdot 0.8 \cdot 0.9 \; .
\end{equation*}

The factor of \num{0.8} is added since utilization above \SI{80}{\percent} often results in routing congestion. Further, the result is multiplied by \num{0.9}, since a sequence overlap is added which decreases the net throughput,  as explained later in Sec. \ref{sec:slo}. 
Previous experiments showed that a clock frequency above \SI{200}{\mega \hertz} often results in timing violations. Thus, in our design-space exploration, we set the limit for $\mathrm{MAC}_\mathrm{sym}$ to the value which corresponds to an approximated throughput of \SI{40}{\giga Bd} with a clock frequency of \SI{200}{\mega \hertz}.

As a result, we can see that most configurations are outperforming the conventional linear equalizer in \ac{ber}. The inferior performance of the conventional equalizer is probably a result of non-linear distortions caused by fiber dispersion, which cannot be compensated by the linear equalizer. Many \ac{ann} configurations even achieve a \ac{ber} of more than one order of magnitude lower than the linear equalizer.

One interesting insight of the design space exploration is the influence of rising $V_p$ on the \ac{ber}. With rising $V_p$, the \ac{ber} stays the same or even improves up to a $V_p$ of \num{8}. This is remarkable since the \ac{mac} operations per symbol are linearly reduced with rising $V_p$, thus throughput raises with $V_p$. Therefore all Pareto optimal points with sufficient performance either correspond to a configuration with $V_p=8$ or $V_p=10$. For higher values of $V_p$, the \ac{ber} increases significantly. 

For our hardware implementation, we select the configuration with the lowest \ac{ber} while satisfying our throughput requirements of \SI{40}{\giga Bd} with a clock frequency of \SI{200}{\mega \hertz}. This configuration is highlighted by the black circle and corresponds to a model with $V_p=8$, $L=3$, $K=9$, and $C=5$. As a next step, this model is quantized with the algorithm described in Sec. \ref{sec:quant}. Our automatic quantization method, achieves an average bit width of \num{9} for weights and of \num{8} for activations, while inputs and outputs are quantized with \num{6} bit. Meanwhile, the \ac{ber} increases only slightly to around \num{3e-4}, which is still one order of magnitude lower than the \ac{ber} of the conventional linear equalizer. Thus, this quantized model is used in the following for final hardware implementation. 

%For quantization, we selected configuration \num{1}: $V_p=10$, $L=3$, $K=9$, $C_\textrm{max}=5$, configuration \num{2}: $V_p=8$, $L=3$, $K=9$, $C_\textrm{max}=5$ and configuration \num{3}: $V_p=10$, $L=3$, $K=15$, $C_\textrm{max}=5$. As shown in Fig. \ref{fig:dse}, quantization increases the \ac{ber} while the number of \ac{mac} operations stays constant. However, as the bit-width of the quantized models is lower, they are much more hardware efficient as compared to full-precision. It can be seen that there is a large gap between quantized and full-precision models in terms of \ac{ber} for configurations \num{1} and \num{3}. For configuration \num{3} the impact of quantization on the hardware performance is neglectable. Therefore, we select this model for implementation, as it achieves an appropriate trade-off between communication performance and hardware complexity. It is to note that due to the flexible topology template, the configurable hardware architecture and \ac{fpga} as a platform, also other configurations can be easily implemented if application requirements change. 

%, likely caused by better generalization





==> chapters/sequence_length_optimization.tex <==
\section{Sequence Length Optimization}
\label{sec:slo}


%\todo{Explain that equalizer is just one application for this approach, but the approach of optimal sequence length per instance can also be applied to other sequences to sequence problems}

%\todo{Hard throughput constraint for minimal sequence length}




As described in Sec. \ref{sec:stream_partitioning}, each input sequence is divided into multiple sub-sequences of length $\ell_\mathrm{inst}$, which are forwarded to the individual instances. However, choosing an optimal $\ell_\mathrm{inst}$ under given application constraints is not straightforward.  On the one side, an overlap of symbols is added at the beginning and the end of each sub-sequence. From this point of view, maximizing $\ell_\mathrm{inst}$ results in the highest throughput since the overall overlap is minimized. On the other side, increasing $\ell_\mathrm{inst}$ raises the latency of the equalizer, which may violate low-latency constraints in applications like high-frequency trading or telemedicine. Thus it is important to choose $\ell_\mathrm{inst}$ carefully, as described in the following. 


\subsection{Timing Model}
\label{sec:timinig_model}
To optimize $\ell_\mathrm{inst}$, we perform a detailed timing analysis of our hardware architecture. First, it is analyzed how many overlap symbols need to be added at the beginning and end of each sequence to compensate for the \ac{ber} increase.  For a \ac{cnn}, the receptive field corresponds to the input symbols taken into account to predict each output. Thus, at the beginning and end of each sequence, half of the receptive field needs to be added as overlap. Based on the formula presented in \cite{Araujo2019}, the number of overlap symbols for our network topology is calculated as
%\begin{equation*}
%    o_\mathrm{sym} = \frac{\sum_{i=1}^{L-1} (K_i - 1) \prod_{j=1}^{i} S_i}{2}  \; .
%\end{equation*}
\begin{equation*}
    o_\mathrm{sym} = \frac{(K - 1) \cdot (1 + V_\mathrm{p} \cdot (L - 1))}{2}  \; .
\end{equation*}
However, this overlap needs to be added before the first \ac{ssm} by the \ac{ogm}, where the stream has a width of $N_\mathrm{i} \cdot V_p$ and has to be dividable by $N_\mathrm{os}$, which equals to \num{2} in our case. Thus, the actual overlap can be calculated as
\begin{equation*}
    o_\mathrm{act} = \mathrm{nextEven}\Bigl(\left \lceil{\frac{o_\mathrm{sym}}{V_\mathrm{p} \cdot N_\mathrm{i}}}\right \rceil \Bigr) \cdot V_\mathrm{p} \cdot N_\mathrm{i}   \; .
\end{equation*}

Therefore, the actual sequence length that needs to be processed including overlap is given as
\begin{equation*}
    \ell_\mathrm{ol} = \ell_{\mathrm{inst}} + 2 \cdot o_\mathrm{act}    \; .
\end{equation*}


As a second step, we analyze how $\ell_\mathrm{ol}$ influences the time to fill the pipeline $t_\mathrm{init}$, afterwards, we explain how this affects the latency of each symbol.

\begin{figure}[h]
	\centering
	%\vspace*{0.18cm}
	%\input{figures/tikz_parallel.tex}
        \includesvg[width=0.9\columnwidth]{figures/latency_new_latex_style.svg}
	\caption{Illustration of the processing time $t_p$ and the time for filling the pipeline $t_\mathrm{init}$ for four \ac{cnn} instances}
        %\vspace*{-4mm}
	\label{fig:latency}
\end{figure}

In Fig. \ref{fig:latency}, it is shown how $\ell_\mathrm{ol}$ and therefore $\ell_\mathrm{inst}$ impact the total time $t$ to process one sequence. This time can be split into $t_\mathrm{init}$ and $t_\mathrm{p}$ and is illustrated for four instances. Since the width of the output streams of an \ac{ssm} is half the width of the input stream and the sequences of length $\ell_\mathrm{ol} / V_\mathrm{p}$ are written alternately to each output, the writing to the second output stream only starts after $\ell_\mathrm{ol} / (2 \cdot V_\mathrm{p})$ clock cycles. Similar behavior can be observed for each stage of the hierarchically arranged \acp{ssm}. Therefore, $t_{\mathrm{init}}$, corresponding to the time where the last \ac{cnn} instance starts processing, is given by
\begin{equation*}
    t_{\mathrm{init}} = \log_2(N_\mathrm{i}) \cdot \frac{\ell_\mathrm{ol}}{2 \cdot V_\mathrm{p} \cdot f_\mathrm{clk}}   \; .
\end{equation*}
Thus, it can be seen that $t_{\mathrm{init}}$ increases linearly with $\ell_{\mathrm{ol}}$ and $\ell_{\mathrm{inst}}$. Is it important to determine $t_\mathrm{init}$, as it directly influences the latency to process one symbol $\lambda_{\mathrm{sym}}$, which is given as the sum of the latency for splitting $\lambda_{\mathrm{spl}}$, processing $\lambda_{\mathrm{pro}}$ and merging $\lambda_{\mathrm{mer}}$. As the \ac{cnn} is fully parallelized and there is no stalling in the merging of streams, $\lambda_{\mathrm{pro}}$ and $\lambda_{\mathrm{mer}}$ are neglectable. In contrast, for splitting, a stream of higher width is converted into streams of lower width, which results in stalling and increased latency. The maximum symbol latency can therefore be approximated as the time $t_\mathrm{init}$ to fill the pipeline:
\begin{equation}
\label{eq:latency}
    \lambda_{\mathrm{sym}} \approx t_{\mathrm{init}} =  \frac{\log_2(N_\mathrm{i}) \cdot \ell_\mathrm{ol}}{2 \cdot V_\mathrm{p} \cdot f_\mathrm{clk}} = \frac{\log_2(N_\mathrm{i}) \cdot (\ell_\mathrm{inst} + 2 \cdot o_\mathrm{act})}{2 \cdot V_\mathrm{p} \cdot f_\mathrm{clk}}\; .
\end{equation}

From (\ref{eq:latency}), it can be seen that higher $\ell_{\mathrm{inst}}$ negatively impacts the symbol latency $\lambda_{\mathrm{sym}}$. From this point of view, it would be beneficial to set $\ell_{\mathrm{inst}}$ as small as possible. 


%Another metric directly influenced by $l_{\mathrm{ol}}$ is the latency to process one symbol $\lambda_{\mathrm{sym}}$, which is given as the sum of the latency for splitting $\lambda_{\mathrm{spl}}$, processing $\lambda_{\mathrm{pro}}$ and merging $\lambda_{\mathrm{mer}}$. As the \ac{cnn} is fully parallelized and there is no stalling in the merging of streams, $\lambda_{\mathrm{pro}}$ and $\lambda_{\mathrm{mer}}$ are neglectable. In contrast, for the splitting, a stream of higher width is converted into streams of lower width, which results in stalling and increased latency. The maximum symbol latency of $\lambda_{\mathrm{spl}}$ is given by the difference of the time where the last symbol of a sequence is written to the \textit{Split Stream} modules and the time when it is read by the \ac{cnn}. Thus the latency for processing one symbol can be approximated as: 
%\begin{equation*}
%    \lambda_{\mathrm{sym}} \approx \lambda_{\mathrm{spl}} \approx  \log_2(N_\mathrm{i}) \cdot \frac{l_\mathrm{ol}}{2 \cdot V_p \cdot f_\mathrm{clk}} - \frac{l_\mathrm{ol}}{V_p \cdot N_\mathrm{i} \cdot f_\mathrm{clk}} = \frac{l_\mathrm{ol}}{V_p \cdot f_\mathrm{clk}} \cdot (\log_2(N_\mathrm{i} - 1) - \frac{1}{N_\mathrm{i}})
%\end{equation*}

%Thus, it can be seen that higher $l_{\mathrm{ol}}$ negatively impacts $t_{\mathrm{init}}$ and the symbol latency $\lambda_{\mathrm{sym}}$. From this point of view, it would be beneficial to set $l_{\mathrm{inst}}$ as small as possible. 

%However, for every sequence of length $l_{\mathrm{inst}}$, an overlap is added to decrease the \ac{ber} at the beginning and end of each sequence. For a \ac{cnn}, the receptive field corresponds to the input symbols taken into account to predict each output. Thus, at the beginning and end of each sequence, half of the receptive field needs to be added as overlap. For our \ac{cnn} topology with $L$ layers, kernel size $K$ and stride $S$, the number of overlap symbols is calculated as: 
%\begin{equation*}
 %   o_\mathrm{sym} = \frac{\sum_{i=1}^{L-1} (K_i - 1) \prod_{j=1}^{i} S_i}{2}
%\end{equation*}
%However, this overlap needs to be added before the first \textit{Split Stream} module, where the stream has a width of $N_\mathrm{i} \cdot V_p$ and has to be dividable by $N_\mathrm{os}$, which is two in our case. Thus, the actual overlap can be calculated as: 
%\begin{equation*}
%    o_\mathrm{act} = \mathrm{nextEven}\Bigl(\left \lceil{\frac{o_\mathrm{sym}}{V_p * N_\mathrm{i}}}\right \rceil \Bigr) \cdot V_p \cdot N_\mathrm{i}
%\end{equation*}

%Therefore, the actual sequence length that needs to be processed including overlap is given as: 
%\begin{equation*}
%    l_\mathrm{ol} = l_{\mathrm{inst}} + 2 \cdot o_\mathrm{act}
%\end{equation*}

However, since $o_\mathrm{act}$ is fixed and is added to each sub-sequence of length $\ell_\mathrm{inst}$, the total number of symbols to process by the \ac{cnn} instances grows with shorter $\ell_\mathrm{inst}$. This is directly reflected in the processing time for one sequence of length $\ell_\mathrm{in}$, which is calculated as
\begin{equation*}
    t_p = \frac{\ell_\mathrm{in}}{\ell_\mathrm{inst} \cdot N_\mathrm{i}} \cdot \frac{\ell_\mathrm{inst} + 2 \cdot o_\mathrm{act}}{V_\mathrm{p} \cdot f_\mathrm{clk}} = \frac{\ell_\mathrm{in}}{N_\mathrm{i} \cdot V_\mathrm{p} \cdot f_\mathrm{clk}} \cdot \Bigl(1 + \frac{2 \cdot o_\mathrm{act}}{\ell_\mathrm{inst}}\Bigr)   \; .
\end{equation*}

The processing time is inversely proportional to the net throughput:
\begin{equation}
\label{eq:net_throughput}
T_\mathrm{net} = \frac{\ell_\mathrm{in}}{t_p} = \frac{N_\mathrm{i} \cdot V_\mathrm{p} \cdot f_\mathrm{clk}}{1 + \frac{2 \cdot o_\mathrm{act}}{\ell_\mathrm{inst}}}   \; .
\end{equation}

Thus, the net throughput grows with larger $\ell_\mathrm{inst}$.
In summary, both the symbol latency $\lambda_{\mathrm{sym}}$ and the throughput $T_\mathrm{net}$ increase with $\ell_\mathrm{inst}$, therefore a trade-off exists when optimizing for throughput and latency. 

%In summary, the time for filling the pipeline $t_\mathrm{init}$ and the symbol latency $\lambda_{\mathrm{sym}}$ increases with larger $l_\mathrm{inst}$, while the processing time $t_p$ is decreased. Based on our timing model for $t_{\mathrm{init}}$ and $t_p$, the total processing time $t$ for one sequence of length $l_\mathrm{in}$ can be derived as: 
%\begin{equation}
%t = t_\mathrm{init} + t_\mathrm{p} =  \log_2(N_\mathrm{i}) \cdot \frac{l_\mathrm{ol}}{2 \cdot V_p \cdot f_\mathrm{clk}} + \frac{l_\mathrm{in}}{N_\mathrm{i} \cdot V_p \cdot f_\mathrm{clk}} \cdot (1 + \frac{2 \cdot o_\mathrm{act}}{l_\mathrm{inst}})
%\end{equation}

%Based on the time for processing $t_p$ also the net throughput $T_\mathrm{net}$ corresponding to the throughput achievable by the equalizer when also considering the overlap symbols of sub-sequences can be calculated as: 
%\begin{equation}
%\label{eq:net_throughput}
%T_\mathrm{net} = \frac{l_\mathrm{in}}{t_p} = \frac{N_\mathrm{i} \cdot V_p \cdot f_\mathrm{c}}{1 + \frac{2 \cdot o_\mathrm{act}}{l_\mathrm{inst}}}
%\end{equation}



\subsection{Optimization Framework}
\label{sec:optimization_framework}

Based on the equations presented in the previous section, we propose a framework to select the best $\ell_\mathrm{inst}$ for the given application requirements. In our case, the throughput is a hard constraint that needs to be satisfied, while latency is an objective we want to minimize. Thus, the framework selects the minimal $\ell_\mathrm{inst}$ which satisfies the throughput requirements. 


\begin{figure}[h]
	\centering
        %\includesvg[width=0.6\columnwidth, inkscapelatex=false]{figures/framework_new.svg}
        \includesvg[width=1\columnwidth]{figures/framework_new_latex_style.svg}
	\caption{Illustration of framework used to optimize sequence length per instance $\ell_\mathrm{inst}$.}
        %\vspace*{-4mm}
	\label{fig:framework}
\end{figure}


%If there is no throughput requirement, $l_\mathrm{inst}$ is chosen to minimize the total processing time. If there is a throughput requirement, the larger value of minimal $l_\mathrm{inst}$ satisfying the requirement and $l_\mathrm{inst}$ reducing runtime, is chosen. This way it is guaranteed that the throughput requirement is satisfied, if possible. 
The framework is shown in Fig. \ref{fig:framework}. Part of the framework, in particular the lookup table which maps the required throughput $T_\mathrm{req}$ to the optimal sub-sequence length $\ell_\mathrm{inst}$, is implemented as a module on the \ac{fpga}. This way, the best $\ell_\mathrm{inst}$ can be selected during runtime individually for each sequence to process. The lookup table is provided by a lookup-table-generator based on the timing model presented in Sec. \ref{sec:timinig_model}. The timing model is derived from a detailed analysis of the hardware architecture and therefore introduced hardware awareness to the LUT-Generator. This information is fed back to the hardware by selecting $\ell_\mathrm{inst}$. This way, our framework is also based on a cross-layer design methodology.



 % validate our  model


%due to the overlap added to each sequence of length $l_{\mathrm{inst}}$ which is needed to achieve low \ac{ber}, the throughput as well as $t_{\mathrm{fp}}$ is impaired by $l_{\mathrm{inst}}$. 





==> makros_own.tex <==


\newcommand{\ffw}{0.7\columnwidth} %{0.285\columnwidth}
\newcommand{\ffh}{0.56\columnwidth} %{0.23\columnwidth}



%\DeclareMathOperator{\fft}{\mathcal{F}}
%\DeclareMathOperator{\ifft}{\mathcal{F}^{-1}}
\newcommand{\fft}[1]{\mathcal{F}\mleft\{#1\mright\}}
\newcommand{\ifft}[1]{\mathcal{F}^{-1}\mleft\{#1\mright\}}

\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator{\Eq}{\mathbb{E}_{q_{\bm{\Phi}}\mlr{\bm{X}\mid \bm{Y}}}}

\newcommand{\elr}{\epsilon_{\mathrm{lr}}} % learning rate
\newcommand{\Nos}{N_{\mathrm{os}}}    % oversampling factor
\newcommand{\Nti}{N_{\mathrm{TI}}}    % number of training iterations
\newcommand{\Nb}{N_{\mathrm{b}}}    % batch-size
\newcommand{\Nd}{N_{\mathrm{d}}}    % number of discr. updates per TI
\newcommand{\Nch}{N_{\mathrm{ch}}}    % number of channels (in CNN)
\newcommand{\Nparam}{N_{\mathrm{param}}}    % number of channels (in CNN)
\newcommand{\Fma}{F_{\mathrm{ma}}}    % filter length of MA (results)
\newcommand{\varN}{\sigma^2_{\mathrm{n}}} % noise variance
\newcommand{\varRefi}{\sigma_\mathrm{ref}^{2}\mlr{i}} % variance of added noise to reference
\newcommand{\Lf}{L_{\mathrm{fiber}}} % fibre length
\newcommand{\adB}{\alpha_{\mathrm{dB}}} % attenuation

%\newcommand{\snr}{\mathrm{SNR}} % fibre length



\newcommand{\lr}[1]{\left(#1\right)}
\newcommand{\mlr}[1]{\mleft(#1\mright)}
\newcommand{\mlrb}[1]{\mleft\{#1\mright\}}

\DeclareMathSymbol{\mlq}{\mathord}{operators}{``}
\DeclareMathSymbol{\mrq}{\mathord}{operators}{`'}

\newcommand{\normDis}[2]{\mathcal{N}\mlr{#1,\,#2}}
\newcommand{\multiNormDis}[3]{\mathcal{N}_{#3}\mlr{#1,\,#2}}
\newcommand{\uniDisN}[2]{\mathcal{U}\mlr{#1,\,#2}}
\newcommand{\multiUniDis}[3]{\mathcal{U}_{#3}\mlr{#1,\,#2}}


% simple implication within math or text
\def\thus{\relax
	\ifmmode
	\implies
	\else
	$\implies$
	\fi}


% Pointing finger for noting important things
\newcommand{\mind}{ \hfill { \textbf{\textcolor{KITred}{\bf \HandLeft} } } }


% colored small box representing end of a proof
\def\endofproof{
	\ifmmode
		\text{\hfill} \textcolor{KITgreen}{\rule{2mm}{2mm}}
	\else
		$\hfill \textcolor{KITgreen}{\rule{2mm}{2mm}}$
	\fi}



%%%%%%%%%%%%%%%%%
% Basic math
%%%%%%%%%%%%%%%%%

% definition sign
\def\defl{:=}

% j and differential calc
\def\j{{\mathrm{j}}}
\def \dd{\, {\mathrm{d}}}

% Real part
\def\real{{\mathrm{Re}}}
\def\imag{{\mathrm{Im}}}

\def\I{{\mathrm{I}}}
\def\Q{{\mathrm{Q}}}

\def\TE{{\mathrm{TE}}}
\def\TM{{\mathrm{TM}}}

\def\H{{\mathrm{H}}}

% Vector notataion
\newcommand\vek[1]{{\bm{#1}}}

% sinc and rect
\newcommand\sinc{{\mathrm{sinc}}}
\newcommand\rect{{\mathrm{rect}}}


% Galois
\def\F{{\mathbb{F}}}


% fields
\def\rz{\ifmmode{\mathbb{R}}%
    \else{\hbox{$\mathbb{R}$}}\fi} 
\def\nz{\ifmmode{\mathbb{N}}%
    \else{\hbox{$\mathbb{N}$}}\fi} 
\def\gz{\ifmmode{\mathbb{Z}}%
   \else{\hbox{$\mathbb{Z}$}}\fi} 
\def\cz{\ifmmode{\mathbb{C}}
    \else{\hbox{$\mathbb{C}$}}\fi}%
\def\qz{\ifmmode{\mathbb{Q}}%
    \else{\hbox{$\mathbb{Q}$}}\fi}%   
\def\K{\ifmmode{\mathbb{K}}%
    \else{\hbox{$\mathbb{K}$}}\fi}%  


% Sets as caligraphic letters
\def\setS{{\mathcal{S}}}
\def\setP{{\mathcal{P}}}
\def\setX{{\mathcal{X}}}
\def\setY{{\mathcal{Y}}}
\def\setZ{{\mathcal{Z}}}
\def\setC{{\mathcal{C}}}
\def\setB{{\mathcal{B}}}





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Probability theory
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Er{\ifmmode{\mathbb{E}}%
    \else{\hbox{$\mathbb{E}$}}\fi}%  
    
\def\V{
	\ifmmode
	{\mathrm{V}}
	\else
	${\mathrm{V}}$
	\fi}    


\def\PO{\mathcal{P}(\Omega)}
\def\sigalg{\mathcal{B}}

\def\NO{N_{\Omega}}
	
% random variables
%\newcommand\rv[1]{{\mathsf{#1}}}
\newcommand\rv[1]{{\uppercase{#1}}}

\def\rvX{\rv{x}}
\def\rvY{\rv{y}}
\def\rvZ{\rv{z}}






%%%%%%%%%%%%%%%%%
% Communications, system theory, and transforms
%%%%%%%%%%%%%%%%%


% Bandpass as Index
\def\bp{{\mathrm{BP}}}


% transform as symbol
\usepackage{trfsigns}

\def\transform{\; \laplace \;}
\def\Transform{\; \Laplace \;}

\newcommand{\vTransform}[1][]{\mbox{\setlength{\unitlength}{0.1em}%
		\begin{picture}(10,20)%
		\put(3,2){\circle{4}}%
		\put(3,4){\line(0,1){12}}%
		\put(3,18){\circle*{4}}%
		\put(10,7){#1}
		\end{picture}%
	}%
}%

\newcommand{\vtransform}[1][]{\mbox{\setlength{\unitlength}{0.1em}%
		\begin{picture}(10,20)%
		\put(3,2){\circle*{4}}%
		\put(3,4){\line(0,1){12}}%
		\put(3,18){\circle{4}}%
		\put(10,7){#1}
		\end{picture}%
	}%
}%     


% Hz and seconds
\newcommand\uHz{\mu{\,\mathrm{Hz}}}
\newcommand\us{{\mu\,\mathrm{s}}}	

% index for indicating sample time
\newcommand\samp{{\mathrm{s}}}

% samples per symbol
\newcommand\sps{{\text{sps}}}

% command for SNR as sans-serif
\newcommand\snr{{\mathsf{SNR}}}

\newcommand\ser{{\mathsf{SER}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Boxes and stuff
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% Command for aligning itemize when using columns; --> add "\AdjustMargins" after \begin{frame}...
\makeatletter
\newcommand*{\AdjustMargins}{%
    \setlength{\beamer@rightmargin}{0em}%
    \setlength{\beamer@leftmargin}{0em}%
}
\makeatother





\newcommand{\myfn}[1]{\footnote{\scriptsize {#1}}}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}


\newcommand\nomarkfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{\scriptsize #1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}



%% \highlight[<colour>]{<stuff>}
%\newcommand{\hi}[2][KITyellow]{
%	\ifmmode
%	{
%		\begin{switch}{#1}
%		\case{white}
%			{
%			\mathchoice%
%			  {\colorbox{#1}{$\displaystyle#2$}}%
%			  {\colorbox{#1}{$\textstyle#2$}}%
%			  {\colorbox{#1}{$\scriptstyle#2$}}%
%			  {\colorbox{#1}{$\scriptscriptstyle#2$}}
%			}
%		\case{KITyellow}
%			{
%				 \mathchoice%
%				  {\colorbox{#1}{$\displaystyle#2$}}%
%				  {\colorbox{#1}{$\textstyle#2$}}%
%				  {\colorbox{#1}{$\scriptstyle#2$}}%
%				  {\colorbox{#1}{$\scriptscriptstyle#2$}}
%			}%
%		\case{KITorange}
%			{
%				 \mathchoice%
%				  {\colorbox{#1}{$\displaystyle#2$}}%
%				  {\colorbox{#1}{$\textstyle#2$}}%
%				  {\colorbox{#1}{$\scriptstyle#2$}}%
%				  {\colorbox{#1}{$\scriptscriptstyle#2$}}
%			}%			
%		\case{KITred}
%			{
%				 \mathchoice%
%				  {\colorbox{#1}{\textcolor{white}{$\displaystyle#2$}}}%
%				  {\colorbox{#1}{\textcolor{white}{$\textstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptscriptstyle#2$}}}
%			}%	
%		\case{KITblue}
%			{
%				 \mathchoice%
%				  {\colorbox{#1}{\textcolor{white}{$\displaystyle#2$}}}%
%				  {\colorbox{#1}{\textcolor{white}{$\textstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptscriptstyle#2$}}}
%			}%
%		\case{KITgreen}
%			{
%				 \mathchoice%
%				  {\colorbox{#1}{\textcolor{white}{$\displaystyle#2$}}}%
%				  {\colorbox{#1}{\textcolor{white}{$\textstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptscriptstyle#2$}}}
%			}%	
%		\case{KITpurple}
%			{
%				 \mathchoice%
%				  {\colorbox{#1}{\textcolor{white}{$\displaystyle#2$}}}%
%				  {\colorbox{#1}{\textcolor{white}{$\textstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptscriptstyle#2$}}}
%			}%	
%		\case{KITcyan}
%			{
%				 \mathchoice%
%				  {\colorbox{#1}{\textcolor{white}{$\displaystyle#2$}}}%
%				  {\colorbox{#1}{\textcolor{white}{$\textstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptstyle#2$}}}
%				  {\colorbox{#1}{\textcolor{white}{$\scriptscriptstyle#2$}}}
%			}%												
%		\end{switch}
%	}
%	\else	
%	{
%	\textcolor{#1}{\textbf #2}
%	}
%	\fi
%	}


% \highlight[<colour>]{<stuff>}
\newcommand{\hi}[2][KITyellow]{
	\ifmmode
	{
		%\tikz[baseline]{\node[fill=#1!50,anchor=base ]{$#2$};}
		 \mathchoice%		
%			{\tikz[baseline]{\node[fill=#1!50,anchor=base ]{$\displaystyle#2$};} }
%			{\tikz[baseline]{\node[fill=#1!50,anchor=base ]{$\textstyle#2$};} }
%			{\tikz[baseline]{\node[fill=#1!50,anchor=base ]{$\scriptstyle#2$};} }
%			{\tikz[baseline]{\node[fill=#1!50,anchor=base ]{$\scriptscriptstyle#2$};} }
			{\colorbox{#1!50}{\textcolor{black}{$\displaystyle#2$}}}%
			{\colorbox{#1!50}{\textcolor{black}{$\textstyle#2$}}}
			{\colorbox{#1!50}{\textcolor{black}{$\scriptstyle#2$}}}
			{\colorbox{#1!50}{\textcolor{black}{$\scriptscriptstyle#2$}}}
	}
	\else
	{
		%\textcolor{#1}{\textbf{#2}}
		{\colorbox{#1!50}{\textcolor{black}{#2}}}
	}
	\fi
	}

	
% Kommando um Hin- und Herschieben zu verhinden
\newcommand{\white}[1]{\textcolor{white}{{#1}}}


% footnotetext that is switched off on the slides given by the first argument
\newcommand{\footnotetextoff}[2]{\alt<#1>{\let\thefootnote\relax\footnotetext{~}}{\footnotetext{\scriptsize #2}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Pages notes and reference
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%%
% KIT-Farben
%
\definecolor{kit-green100}{rgb}{0,.59,.51}
\definecolor{kit-green70}{rgb}{.3,.71,.65}
\definecolor{kit-green50}{rgb}{.50,.79,.75}
\definecolor{kit-green30}{rgb}{.69,.87,.85}
\definecolor{kit-green15}{rgb}{.85,.93,.93}
\definecolor{KITgreen}{rgb}{0,.59,.51}

\definecolor{KITpalegreen}{RGB}{130,190,60}
\colorlet{kit-maigreen100}{KITpalegreen}
\colorlet{kit-maigreen70}{KITpalegreen!70}
\colorlet{kit-maigreen50}{KITpalegreen!50}
\colorlet{kit-maigreen30}{KITpalegreen!30}
\colorlet{kit-maigreen15}{KITpalegreen!15}

\definecolor{KITblue}{rgb}{.27,.39,.66}
\definecolor{kit-blue100}{rgb}{.27,.39,.67}
\definecolor{kit-blue70}{rgb}{.49,.57,.76}
\definecolor{kit-blue50}{rgb}{.64,.69,.83}
\definecolor{kit-blue30}{rgb}{.78,.82,.9}
\definecolor{kit-blue15}{rgb}{.89,.91,.95}

\definecolor{KITyellow}{rgb}{.98,.89,0}
\definecolor{kit-yellow100}{cmyk}{0,.05,1,0}
\definecolor{kit-yellow70}{cmyk}{0,.035,.7,0}
\definecolor{kit-yellow50}{cmyk}{0,.025,.5,0}
\definecolor{kit-yellow30}{cmyk}{0,.015,.3,0}
\definecolor{kit-yellow15}{cmyk}{0,.0075,.15,0}

\definecolor{KITorange}{rgb}{.87,.60,.10}
\definecolor{kit-orange100}{cmyk}{0,.45,1,0}
\definecolor{kit-orange70}{cmyk}{0,.315,.7,0}
\definecolor{kit-orange50}{cmyk}{0,.225,.5,0}
\definecolor{kit-orange30}{cmyk}{0,.135,.3,0}
\definecolor{kit-orange15}{cmyk}{0,.0675,.15,0}

\definecolor{KITred}{rgb}{.63,.13,.13}
\definecolor{kit-red100}{cmyk}{.25,1,1,0}
\definecolor{kit-red70}{cmyk}{.175,.7,.7,0}
\definecolor{kit-red50}{cmyk}{.125,.5,.5,0}
\definecolor{kit-red30}{cmyk}{.075,.3,.3,0}
\definecolor{kit-red15}{cmyk}{.0375,.15,.15,0}

\definecolor{KITlilac}{RGB}{160,0,120}
\colorlet{kit-lila100}{KITlilac}
\colorlet{kit-lila70}{KITlilac!70}
\colorlet{kit-lila50}{KITlilac!50}
\colorlet{kit-lila30}{KITlilac!30}
\colorlet{kit-lila15}{KITlilac!15}

\definecolor{KITcyanblue}{RGB}{80,170,230}
\colorlet{kit-cyanblue100}{KITcyanblue}
\colorlet{kit-cyanblue70}{KITcyanblue!70}
\colorlet{kit-cyanblue50}{KITcyanblue!50}
\colorlet{kit-cyanblue30}{KITcyanblue!30}
\colorlet{kit-cyanblue15}{KITcyanblue!15}


% %\definecolor{ALUColor1}{rgb}{0,0.4470,0.7410}
% %\definecolor{ALUColor2}{rgb}{0.8500,0.3250,0.0980}
% \definecolor{ALUColor3}{rgb}{0.9290,0.6940,0.1250}
% %\definecolor{ALUColor4}{rgb}{0.4940,0.1840,0.5560}
% %\definecolor{ALUColor5}{rgb}{0.4660,0.6740,0.1880}
% % colorbrewer 6-class Set1 (qualitative)
% \definecolor{ALUColor1}{RGB}{77,175,74} % colorbrewer 3 (CMA)
% \definecolor{ALUColor2}{RGB}{228,26,28} % colorbrewer 1 (VAE-LE)
% %\definecolor{ALUColor3}{RGB}{77,175,74}
% \definecolor{ALUColor4}{RGB}{55,126,184} % colorbrewer 2 (VAE-NN)
% \definecolor{ALUColor6}{RGB}{152,78,163}

% \definecolor{ALUColor5}{RGB}{255,127,0}
% \definecolor{ALUColor7}{rgb}{0.6350,0.0780,0.1840}

% \definecolor{ALUColor1_70}{rgb}{0,0.3129,0.5187}
% \definecolor{ALUColor2_70}{rgb}{0.5950,0.2275,0.0686}
% %\definecolor{ALUColor2_light}{rgb}{1,0.3823529411,0.115294117624}
% \definecolor{ALUColor2_light}{RGB}{226,97,99}

% \definecolor{ALUColor1_dark}{RGB}{14, 108, 1} 
% \definecolor{ALUColor1_light}{RGB}{0,104,55} 
% \definecolor{ALUColor1_blue}{RGB}{11, 196, 86} 

% % colorbrewer2.0 7-class Set3 (qualitative) --- too bright?
% \definecolor{ALUColor4}{RGB}{141,211,199}   % ganLin
% \definecolor{ALUColor3}{RGB}{255,255,179}   % supLin
% \definecolor{ALUColor7}{RGB}{190,186,218}   % woEq
% \definecolor{ALUColor2}{RGB}{251,128,114}   % sup
% \definecolor{ALUColor5}{RGB}{128,177,211}   % lms
% \definecolor{ALUColor6}{RGB}{253,180,98}    % VNLE
% \definecolor{ALUColor1}{RGB}{179,222,105}   % gan

% % colorbrewer2.0: mix of 5-class RdYlGn and Spectral (diverging)
% \definecolor{ALUColor4}{RGB}{43,131,186}   % ganLin
% \definecolor{ALUColor3}{RGB}{255,255,191}   % supLin
% \definecolor{ALUColor7}{RGB}{166,217,106}   % woEq
% \definecolor{ALUColor2}{RGB}{253,174,97}   % sup
% \definecolor{ALUColor5}{RGB}{171,221,164}   % lms
% \definecolor{ALUColor6}{RGB}{26,150,65}    % VNLE
% \definecolor{ALUColor1}{RGB}{215,25,28}   % gan

% % colorbrewer2.0: 7-class paired (qualitative)
% \definecolor{ALUColor4}{RGB}{251,154,153}   % ganLin
% \definecolor{ALUColor3}{RGB}{166,206,227}   % supLin
% \definecolor{ALUColor7}{RGB}{253,191,111}   % woEq
% \definecolor{ALUColor2}{RGB}{31,120,180}   % sup
% \definecolor{ALUColor5}{RGB}{51,160,44}   % lms
% \definecolor{ALUColor6}{RGB}{178,223,138}    % VNLE
% \definecolor{ALUColor1}{RGB}{227,26,28}   % gan

% colorbrewer2.0: 9-class Set1 (qualitative)
\definecolor{ALUColor4}{RGB}{255,127,0}   % ganLin
\definecolor{ALUColor3}{RGB}{77,175,74}   % supLin
\definecolor{ALUColor7}{RGB}{153,153,153}   % woEq
\definecolor{ALUColor2}{RGB}{55,126,184}   % sup
\definecolor{ALUColor5}{RGB}{152,78,163}   % lms
\definecolor{ALUColor6}{RGB}{166,86,40}    % VNLE
\definecolor{ALUColor1}{RGB}{228,26,28}   % gan

% colorbrewer2.0: 4-class OrRd (sequential)
\definecolor{ALUColor1v}{RGB}{253,204,138}   % ganLin
\definecolor{ALUColor2v}{RGB}{252,141,89}   % supLin
\definecolor{ALUColor3v}{RGB}{215,48,31}   % woEq


